Vision-based Vineyard Navigation Solution with Automatic Annotation

Autonomous navigation is the key to achieving the full automation of agricultural research and production management (e.g., disease management and yield prediction) using agricultural robots. In this paper, we introduced a vision-based autonomous navigation framework for agriculture robots in trellised cropping systems such as vineyards. To achieve this, we proposed a novel learning-based method to estimate the path traversibility heatmap directly from an RGB-D image and subsequently convert the heatmap to a preferred traversal path. An automatic annotation pipeline was developed to form a training dataset by projecting RTK GPS paths collected during the first setup in a vineyard in corresponding RGB-D images as ground-truth path annotations, allowing a fast model training and fine-tuning without costly human annotation. The trained path detection model was used to develop a full navigation framework consisting of row tracking and row switching modules, enabling a robot to traverse within a crop row and transit between crop rows to cover an entire vineyard autonomously. Extensive field trials were conducted in three different vineyards to demonstrate that the developed path detection model and navigation framework provided a cost-effective, accurate, and robust autonomous navigation solution in the vineyard and could be generalized to unseen vineyards with stable performance.

==> dump/related-ref.tex <==
Visual odometry performs poorly for repetitive patterns like crop fields.

\begin{itemize}
    \item \cite{sivakumar2021learned}
    \begin{itemize}
        \item canopy farm robots. truncated resnet-18 output robot heading and placement (distance ratio) in row then compute row center. Just use RGB camera.
        \item works well
        \item needs manual annotation and must be straight line, doesn't do row switching, see failure cases.
    \end{itemize} 
    %%%%%
    \item \cite{martini2022position}
    \begin{itemize}
        \item Use RL
        \item 
        \item Test in simulation only.
    \end{itemize}
    %%%%%%%
    \item \cite{aghi2021deep}
    \begin{itemize}
        \item a custom-trained segmentation
network and a low-range RGB-D camera. Generate  the segmentation maps. Test in simulation and real world data. Take pretrained on image net initialization. IoU loss function. THey find empty columns, compute linear and angular velocity from here,
        \item manual annotation + Gaussian mixture. dataset=1538. THe controller angular velocity proportional to the quadratic of center of cluster from middle of of image. But this is not in BeV. Velocity is similar. Sensitive to field structure whether has multiple holes. if end of row
    \end{itemize}

    \item \cite{ahmadi2020visual}
    \begin{itemize}
        \item Do row switching using front and back cams. row-crop field. ROw crop detection. Extract vegetation mask (non DL) compute center of cluster/connected components. Did line fitting.
        \item  use a fairly straight-forward approach to detect the crop
rows as our main focus has been on the design of the visual
servoing controller and more sophisticated detection methods
are easily implementable. works only for simple structure. Test on row real robot 15m only (ours is 180). Row switching required stepping on the plants.
        \item
    \end{itemize}

    %%%%%%%%%%
    \item \cite{ahmadi2022towards}
    \begin{itemize}
        \item Row crops. ROw switching (but also row crops). omniwheels, four-wheel steering and driven (4WS/4WD). the side-ways
movement of BonnBot-I allowing easier transitions. Use SIFT to detect rows for multi row switching. FOr the line tracking : vegetation mask+ sliding window
        \item 
    \end{itemize}
\end{itemize}

GPS based line tracking line following.
Why we dont prefer:  cost, setup, availability, signal loss, 

LiDAR based
 
Vision based Line tracking. line following, moving in row.
Non DL
DL
RL based.
BUt most work focus primarily on line tracking...


Row switching.
Describe the row switching
But this only works for row crops. 

